YBa$_2$Cu$_3$O$_7$ nano-constriction Josephson junctions and SQUIDs fabricated by focused helium-ion-beam irradiation

By focused $30\,\mathrm{keV}$ He ion beam irradiation, epitaxially grown YBa$_2$Cu$_3$O$_7$ (YBCO) thin films can be driven from the superconducting to the insulating state with increasing irradiation dose. A properly chosen dose suppresses superconductivity down to $4\,\mathrm{K}$, while crystallinity is still preserved. With this approach we create areas of normal-conducting YBCO that can be used to define resistively shunted constriction-type Josephson junctions (cJJs) on the nanometer scale. We also demonstrate that the fabricated cJJs can be incorporated in direct current superconducting quantum interference devices and can be used as detector junctions in THz antennas.

==> MyMc.tex <==
%%% This is 'MyMc.tex' v3.00
%%% LaTeX macros for frequently used abbreviations
%%% 13.12.2011 by Edward Goldobin <gold@uni-tuebingen.de>

\RequirePackage{xspace}

%stupid macros like \ie, \eg, \etc
\newcommand{\ie}{\textit{i.e.}\xspace}
\newcommand{\ia}{\textit{i.a.}\xspace}
\newcommand{\eg}{\textit{e.g.}\xspace}
\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\cf}{\textit{cf.}\xspace}
\newcommand{\vs}{\textit{vs.}\xspace}
\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\viz}{\textit{viz.}\xspace}
%\newcommand{\etal}{\textit{et~al.}\xspace}
\newcommand{\lhs}{l.h.s.\@\xspace}
\newcommand{\rhs}{r.h.s.\@\xspace}
%German versions:
\renewcommand{\dh}{d.h.\xspace}
\newcommand{\zB}{z.B.\xspace}
\newcommand{\ua}{u.a.\xspace}
\newcommand{\vgl}{vgl.\xspace}
\newcommand{\usw}{usw.\xspace}
\newcommand{\bzw}{bzw.\xspace}


\newcommand{\mum}{\ensuremath{\mathrm{\mu m}}}
\newcommand{\degree}{\ensuremath{^\circ}\xspace}

%units
\newcommand{\units}[2][\,]{\ensuremath{#1\mathrm{#2}}}
\newcommand{\Ohm}{\ensuremath{\Omega}}

% Convenient ratios and (partial) derivatives
%
%big \frac is called \ratio.
%usage: \ratio{a}{b}
\newcommand{\ratio}[2]{\displaystyle\frac{#1}{#2}}
%usage: \fracd{y}{x} produces fraction dy/dx.
%usage with optional argument: \fracd[2]{y}{x} produces 2nd derivative
\newcommand{\fracd}[3][]{\displaystyle\frac{d^{#1}#2}{d#3^{#1}}}
%usage: \fracp{y}{x} produces partial derivatice dy/dx.
%usage with optional argument: \fracp[2]{y}{x} produces 2nd order partial derivative
\newcommand{\fracp}[3][]{\displaystyle\frac{\partial^{#1}#2}{\partial#3^{#1}}}
%mixed only for 2 vars
% \fracpii{f}{x}{y}
\newcommand{\fracpii}[3]{\displaystyle\frac{\partial^{2}#1}{\partial#2\partial#3}}
%mixed derivatives are not implemented yet :-(
\newcommand{\fracpmix}[3]{\displaystyle\frac{\partial^2#1}{\partial#2\partial#3}}
%ideally: \fracp*{f}{x^2,y,z} or \fracp*{f}{x,x,y,z}
%usage: \divp{f}{x} produces partial derivative df/dx.
%usage with optional argument: \divp[2]{f}{x} produces 2nd order partial derivative
\newcommand{\divp}[3][]{{\partial^{#1}#2}/{\partial#3^{#1}}}

%Averaging macros:
%
%usage1: \av{V} - averaged V
%usage2: \av[x]{V} - V averaged with respect to x
\newcommand{\av}[2][]{\ensuremath{\left\langle#2\right\rangle_{#1}}\xspace}
%usage: \mean{u} - produced bar over the argument
\newcommand{\mean}[1]{\ensuremath{\overline{#1}}\xspace}
\newcommand{\dev}[2][]{\ensuremath{\widetilde{#2}_{#1}}\xspace}

\newcommand{\bra}[1]{\ensuremath{\left\langle #1\right|}\xspace}
\newcommand{\ket}[1]{\ensuremath{\left| #1\right\rangle}\xspace}
\newcommand{\braket}[1]{\ensuremath{\left\langle #1\right\rangle}\xspace}

%shorter braces:
\newcommand\braces[1]{\rbraces{#1}}
\newcommand\rbraces[1]{\ensuremath{\left( #1\right)}}
\newcommand\sbraces[1]{\ensuremath{\left[ #1\right]}}
\newcommand\fbraces[1]{\ensuremath{\left\{ #1\right\}}}
\newcommand\tbraces[1]{\ensuremath{\left< #1\right>}}
\newcommand\abraces[1]{\ensuremath{\left| #1\right|}}
%braced frac
\newcommand\rbfrac[2]{\ensuremath{\left( \frac{#1}{#2}\right)}}
\newcommand\sbfrac[2]{\ensuremath{\left[ \frac{#1}{#2}\right]}}
\newcommand\fbfrac[2]{\ensuremath{\left\{\frac{#1}{#2}\right\}}}
\newcommand\tbfrac[2]{\ensuremath{\left< \frac{#1}{#2}\right>}}
\newcommand\abfrac[2]{\ensuremath{\left| \frac{#1}{#2}\right|}}

%3D vectors with comma-separated coords
%usage: \VEC(1,1,0)
\def\innervector(#1,#2,#3){\begin{matrix}#1\\#2\\#3\end{matrix}}
\def\VEC#1{\braces{\negthinspace\innervector(#1)}}
\def\sVEC#1{\sbraces{\innervector(#1)}}
\def\fVEC#1{\fbraces{\negthinspace\innervector(#1)}}
\def\aVEC#1{\abraces{\innervector(#1)}}
\def\AVEC#1{\abraces{\abraces{\innervector(#1)}}}


%%
%% Freq used math symbols
%%

%Special (Elliptic) fns
\newcommand{\am}{\mathop{\mathrm{am}}\nolimits}
% \newcommand{\dn}{\mathop{\mathrm{dn}}\nolimits}
\newcommand{\sn}{\mathop{\mathrm{sn}}\nolimits}
\newcommand{\cn}{\mathop{\mathrm{cn}}\nolimits}
\newcommand{\gd}{\mathop{\mathrm{gd}}\nolimits}
\newcommand{\E} {\mathop{\mathrm{E}}\nolimits}
\newcommand{\F} {\mathop{\mathrm{F}}\nolimits}
\newcommand{\K} {\mathop{\mathrm{K}}\nolimits}
\newcommand{\J}[1][] {\mathop{\mathrm{J_{#1}}}\nolimits}
\newcommand{\Ai} {\mathop{\mathrm{Ai}}\nolimits}
\newcommand{\Bi} {\mathop{\mathrm{Bi}}\nolimits}

%Other fns
\newcommand{\asinh}{\mathop{\mathrm{Arsinh}}\nolimits}
\newcommand{\acosh}{\mathop{\mathrm{Arcosh}}\nolimits}
\newcommand{\atanh}{\mathop{\mathrm{Artanh}}\nolimits}
\newcommand{\acot}{\mathop{\mathrm{acot}}\nolimits}
\newcommand{\sech}{\mathop{\mathrm{sech}}\nolimits}

\newcommand{\sgn}{\mathop{\mathrm{sgn}}\nolimits}
\newcommand{\floor}{\mathop{\mathrm{floor}}\nolimits}
\newcommand{\ceil}{\mathop{\mathrm{ceil}}\nolimits}
\newcommand{\const}{\mathop{\mathrm{const}}\nolimits}

%%
%% Complex numbers {
%%
\renewcommand{\Re}{\mathop{\mathrm{Re}}\nolimits}
\renewcommand{\Im}{\mathop{\mathrm{Im}}\nolimits}
%\newcommand{\arg}{\mathop{\mathrm{arg}}\nolimits}
%imaginary i and j
\newcommand{\ii}{\ensuremath{\mathrm{i}}}
%\newcommand{\ij}{\ensuremath{\mathrm{i}}}
%%}

%some symbols that should be Roman to stress that they are not (parts of)variables
% \newcommand{\dd}{\ensuremath{\,\mathrm{d}}}
\newcommand{\ee}{\ensuremath{\mathrm{e}}\xspace}

%\newcommand{\O}{\mathop{\mathrm{O}}\nolimits} %of the order of
%\newcommand{\d}{\mathop{\mathrm{d}}} %d in integrad dx, dy, dz

%\newcommand{\Det}{\mathop{\mathrm{det}}\nolimits}
%\newcommand{\Tr}{\mathop{\mathrm{Tr}}\nolimits}

\newcommand{\qstate}[1]{\ensuremath{\left\lvert\state{#1}\right\rangle}}
\newcommand{\rot}{\mathop\mathrm{\mathbf{rot}}\nolimits}
\newcommand{\grad}{\mathop\mathbf{{\rm grad}}\nolimits}
%\newcommand{\div}{\mathop{{\rm div}}\nolimits}

%Freq used materials
\RequirePackage{xspace}
\newcommand{\YBCO}[1][7]{YBa$_2$Cu$_3$O$_{#1}$\xspace}
\newcommand{\LBCO}[1][x]{La$_{2-#1}$Ba$_#1$CuO$_4$\xspace}
\newcommand{\BSCCO}{Bi$_2$Sr$_2$Ca$_1$Cu$_2$O$_{8}$\xspace}
\newcommand{\NBCO}[1][x]{NdBa$_2$Cu$_3$O$_{7-#1}$\xspace}
\newcommand{\TBCO}{Tl$_2$Ba$_2$CuO$_6$\xspace}
\newcommand{\HBCO}{HgBa$_2$CuO$_6$\xspace}
\newcommand{\NCCO}{Nd$_{2-x}$Ce$_x$CuO$_4$\xspace}
\newcommand{\PCCO}{Pr$_{2-x}$Ce$_x$CuO$_4$\xspace}
\newcommand{\LCMO}[1][x]{La$_{1-#1}$Ca$_x$MnO$_3$\xspace}
\newcommand{\STO}{SrTiO$_3$\xspace}
\newcommand{\LSAT}{(LaAlO$_3$)$_3$(Sr$_2$AlTaO$_6$)$_7$\xspace}
\newcommand{\CeO}{CeO$_2$\xspace}
\newcommand{\MgB}{MgB$_2$\xspace}
\newcommand{\OrgIJJ}{$\kappa$-(BEDT-TTF)$_2$Cu(NCS)$_2$\xspace}

%%%
%%% Frequently used physics notations
%%%

%technology definitions
\newcommand{\NbAlOxNb}{Nb-AlO$_x$-Nb\xspace}
\newcommand{\TechNb}{Nb-AlO$_x$-Nb\xspace}
\newcommand{\TechYBCONb}{YBCO-Nb\xspace}
%
\newcommand{\SIS}{\ensuremath{\mathrm{S|I|S}}\xspace}
\newcommand{\SNS}{\ensuremath{\mathrm{S|N|S}}\xspace}
\newcommand{\SFS}{\ensuremath{\mathrm{S|F|S}}\xspace}
\newcommand{\SIFS}{S$|$I$|$F$|$S\xspace}
\newcommand{\SfiS}{S$|$FI$|$S\xspace}
%\newcommand{\SJS}{\ensuremath{\mathrm{S-FI-S}}\xspace}



%just shortcuts
%\newcommand{\HS}{\ensuremath{{\cal H}}}
\newcommand{\Heavyside}{\mathop{\mathrm{H}}\nolimits}
%\newcommand{\G}{\ensuremath{{\cal G}}}
\newcommand{\Dx}{\ensuremath{{\Delta x}}}
\newcommand{\dx}{\ensuremath{{\delta x}}}
\newcommand{\Dw}{\ensuremath{{\Delta w}}}
\newcommand{\D}[1]{\ensuremath{{\Delta #1}}}
%\newcommand{\d}[1]{\ensuremath{{\delta #1}}}

\newcommand{\kB}{\ensuremath{k_\mathrm{B}}}
\newcommand{\kBT}{\ensuremath{k_\mathrm{B}T}}

%\iffalse%{
\RequirePackage{amssymb}

% macros for showing/hiding corrections
%usage and result for ShowCorrection=true/false:
%\new{text} blue/normal
%\old{text} red strikedout/hidden
%\note{text} gray/hidden

\RequirePackage{ifthen}
\RequirePackage{color}
\usepackage[normalem]{ulem}
\newboolean{ShowCorrections}
\setboolean{ShowCorrections}{true}%<-- set here show/notshow corrections

%%%Reduction/Corrections/notes macros
\DeclareRobustCommand{\new}[1]{%
  \ifthenelse{\boolean{ShowCorrections}}{\textcolor[rgb]{0,0,1}{#1}}{#1}%
}
\DeclareRobustCommand{\old}[1]{%
  \ifthenelse{\boolean{ShowCorrections}}{\textcolor[rgb]{1,0,0}{\sout{#1}}}{#1}%
}
\DeclareRobustCommand{\note}[1]{%
  \ifthenelse{\boolean{ShowCorrections}}{\textcolor{gray}{#1}}{}
}%

%select hard references to make them noticable
\newcommand{\hardref}[1]{\textcolor{orange}{#1}}

%%
%% Not allowed stuff
%%

%state command which may not translate correctly
\newcommand{\stat}[1]{\state{#1}}

%%tth:\def\relax{}
%%tth:\def\message#1{}

%\tracingmacros=2
%%%%%%%%%%

\def\state#1{\ensuremath{\stt#1.}}
\def\stt#1{%
\if#1.
\let\next=\relax
\else
  \if#1u
    \upharpoonleft%\uparrow
  \else\if#1d
    \downharpoonleft%\downarrow
  \else\if#1U
    \upharpoonright%\Uparrow
  \else\if#1D
    \downharpoonright%\Downarrow
  \else\if#1F
    \Uparrow
  \else\if#1A
    \Downarrow
  \else\if#1s
    \uparrow
  \else\if#1a
    \downarrow
  \else\if#1r
    \rightarrow
  \else\if#1l
    \leftarrow
  \else\if#1R
    \Rightarrow
  \else\if#1L
    \Leftarrow
  \else\if#1>
    \longrightarrow
  \else\if#1<
    \longleftarrow
  \else\if#1
  \relax
  \else
  ?\message{Unknown symbol #1 in the argument of macro state}
  \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
\let\next=\stt
\fi
\next
}

\def\spins#1{\ensuremath{\spn#1.}}
\def\spn#1{%
\if#1.
\let\next=\relax
\else
  \if#1u
    \uparrow
  \else\if#1d
    \downarrow
  \else\if#1U
    \Uparrow
  \else\if#1D
    \Downarrow
  \else\if#1r
    \rightarrow
  \else\if#1l
    \leftarrow
  \else\if#1R
    \Rightarrow
  \else\if#1L
    \Leftarrow
  \else\if#1>
    \longrightarrow
  \else\if#1<
    \longleftarrow
  \else\if#1h
    \leftrightarrow
  \else\if#1v
    \updownarrow
  \else\if#1_%
    \;\;
  \else\if#1,%
    \,
  \else\if#1;%
    \;
  \else\if#1|%
    \vdots%
  \else\if#1-%
    \hdots%
  \else\if#1
  \relax
  \else
  ?\message{Unknown symbol #1 in the argument of macro spins}
  \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
\let\next=\spn
\fi
\next
}

%usage: \hstruct{Nb|Al|Nb}
%at the moment cannot accept math or lower indices. :-(
\def\hstruct#1{%
\let\accu=\relax%
\hstruc#1.%
\accu
}
\def\hstruc#1{%
\if#1.%end?
\let\next=\relax
\else
  \if#1|%
    \let\accu=\accu$|$%
%  \else\if#1
%    \relax
  \else
    \let\accu=\accu #1%\message{Unknown symbol #1 in the argument of macro \hstruc}
  \fi%\fi
  \let\next=\hstruc
\fi
\next
}


\newcounter{CurrTimeHH}\newcounter{CurrTimeMM}
\newcommand{\CurrTime}{%
  \setcounter{CurrTimeHH}{\time/60}%
  \setcounter{CurrTimeMM}{\time - \value{CurrTimeHH}*60}%
  \ifthenelse{\value{CurrTimeHH}<10}{0}{}\theCurrTimeHH:%
  \ifthenelse{\value{CurrTimeMM}<10}{0}{}\theCurrTimeMM%
}



